Prolog for Verification, Analysis and Transformation Tools

This article examines the use of the Prolog language for writing verification, analysis and transformation tools. Guided by experience in teaching and the development of verification tools like ProB or specialisation tools like ECCE and LOGEN, the article presents an assessment of various aspects of Prolog and provides guidelines for using them. The article shows the usefulness of a few key Prolog features. In particular, it discusses how to deal with negation at the level of the object programs being verified or analysed.

==> eptcsdata.tex <==
\providecommand{\firstpage}{80}
\providecommand{\publicationstatus}{L. Fribourg and M. Heizmann (Eds.): VPT/HCVS 2020\\
EPTCS 320, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.320.6}{10.4204/EPTCS.320.6}}
\pdfoutput=1

